Tracking UWB Devices Through Radio Frequency Fingerprinting Is Possible

Ultra-wideband (UWB) is a state-of-the-art technology designed for applications requiring centimeter-level localization. Its widespread adoption by smartphone manufacturer naturally raises security and privacy concerns. Successfully implementing Radio Frequency Fingerprinting (RFF) to UWB could enable physical layer security, but might also allow undesired tracking of the devices. The scope of this paper is to explore the feasibility of applying RFF to UWB and investigates how well this technique generalizes across different environments. We collected a realistic dataset using off-the-shelf UWB devices with controlled variation in device positioning. Moreover, we developed an improved deep learning pipeline to extract the hardware signature from the signal data. In stable conditions, the extracted RFF achieves over 99% accuracy. While the accuracy decreases in more changing environments, we still obtain up to 76% accuracy in untrained locations.

==> Sections/experimental_set_up_figure.tex <==
%\documentclass[10pt]{article}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.15}
%\usepackage{mathrsfs}
%\usetikzlibrary{arrows}
%\pagestyle{empty}


\definecolor{uuuuuu}{rgb}{0.26666666666666666,0.26666666666666666,0.26666666666666666}
\definecolor{zzttqq}{rgb}{0.6,0.2,0}
\definecolor{ududff}{rgb}{0.30196078431372547,0.30196078431372547,1}
\begin{tikzpicture}[line cap=round,line join=round,>=triangle 45,x=0.1cm,y=1cm, scale=0.2]
\begin{axis}[
x=1cm,y=1cm,
axis lines=none,
ymajorgrids=false,
xmajorgrids=false,
xmin=-1,
xmax=33,
ymin=-18,
ymax=18,
xtick={-10,-5,...,65},
ytick={-20,-15,...,20},]
\clip(-12.723284590217933,-21.19884450414584) rectangle (67.52610567534713,24.84502889234998);
\fill[line width=2pt,color=zzttqq,fill=zzttqq,fill opacity=0.10000000149011612] (0,2) -- (0,0) -- (0.2506664671286085,-1.9842294026289462) -- (0.7480462414583151,-3.921395724886205) -- (1.4842953468276683,-5.780948696662703) -- (2.447802695031097,-7.5335620567504264) -- (3.62337319961604,-9.151596045500318) -- (4.992467411473415,-10.609533300343136) -- (6.533493897024991,-11.884381279840513) -- (8.222149748029015,-12.956034869798504) -- (10.03180385296105,-13.807593452928646) -- (11.933916885551353,-14.425627441678541) -- (13.898491387008725,-14.80039007084999) -- (15.894544843865264,-14.925971109908616) -- (17.890598300721805,-14.80039007084999) -- (19.855172802179176,-14.425627441678543) -- (21.757285834769476,-13.807593452928648) -- (23.566939939701516,-12.956034869798504) -- (25.255595790705538,-11.884381279840516) -- (26.796622276257118,-10.609533300343136) -- (28.165716488114484,-9.151596045500321) -- (29.34128699269943,-7.533562056750428) -- (30.30479434090286,-5.780948696662704) -- (31.041043446272212,-3.9213957248862084) -- (31.538423220601924,-1.9842294026289484) -- (31.78908968773053,0) -- (31.78908968773053,2) -- (31.53842322060192,3.9842294026289498) -- (31.041043446272212,5.92139572488621) -- (30.30479434090286,7.780948696662704) -- (29.34128699269943,9.53356205675043) -- (28.16571648811449,11.151596045500318) -- (26.796622276257114,12.609533300343138) -- (25.255595790705538,13.884381279840516) -- (23.56693993970151,14.956034869798508) -- (21.757285834769483,15.807593452928646) -- (19.85517280217918,16.425627441678543) -- (17.890598300721802,16.80039007084999) -- (15.894544843865262,16.925971109908616) -- (13.898491387008722,16.80039007084999) -- (11.93391688555136,16.425627441678543) -- (10.031803852961055,15.80759345292865) -- (8.222149748029018,14.956034869798504) -- (6.533493897024989,13.884381279840513) -- (4.992467411473411,12.609533300343134) -- (3.6233731996160383,11.151596045500312) -- (2.4478026950311005,9.53356205675043) -- (1.48429534682767,7.780948696662706) -- (0.7480462414583151,5.921395724886204) -- (0.25066646712860674,3.9842294026289435) -- cycle;
\draw [line width=2pt,color=zzttqq] (0,2)-- (0,0);
\draw [line width=2pt,color=zzttqq] (0,0)-- (0.2506664671286085,-1.9842294026289462);
\draw [line width=2pt,color=zzttqq] (0.2506664671286085,-1.9842294026289462)-- (0.7480462414583151,-3.921395724886205);
\draw [line width=2pt,color=zzttqq] (0.7480462414583151,-3.921395724886205)-- (1.4842953468276683,-5.780948696662703);
\draw [line width=2pt,color=zzttqq] (1.4842953468276683,-5.780948696662703)-- (2.447802695031097,-7.5335620567504264);
\draw [line width=2pt,color=zzttqq] (2.447802695031097,-7.5335620567504264)-- (3.62337319961604,-9.151596045500318);
\draw [line width=2pt,color=zzttqq] (3.62337319961604,-9.151596045500318)-- (4.992467411473415,-10.609533300343136);
\draw [line width=2pt,color=zzttqq] (4.992467411473415,-10.609533300343136)-- (6.533493897024991,-11.884381279840513);
\draw [line width=2pt,color=zzttqq] (6.533493897024991,-11.884381279840513)-- (8.222149748029015,-12.956034869798504);
\draw [line width=2pt,color=zzttqq] (8.222149748029015,-12.956034869798504)-- (10.03180385296105,-13.807593452928646);
\draw [line width=2pt,color=zzttqq] (10.03180385296105,-13.807593452928646)-- (11.933916885551353,-14.425627441678541);
\draw [line width=2pt,color=zzttqq] (11.933916885551353,-14.425627441678541)-- (13.898491387008725,-14.80039007084999);
\draw [line width=2pt,color=zzttqq] (13.898491387008725,-14.80039007084999)-- (15.894544843865264,-14.925971109908616);
\draw [line width=2pt,color=zzttqq] (15.894544843865264,-14.925971109908616)-- (17.890598300721805,-14.80039007084999);
\draw [line width=2pt,color=zzttqq] (17.890598300721805,-14.80039007084999)-- (19.855172802179176,-14.425627441678543);
\draw [line width=2pt,color=zzttqq] (19.855172802179176,-14.425627441678543)-- (21.757285834769476,-13.807593452928648);
\draw [line width=2pt,color=zzttqq] (21.757285834769476,-13.807593452928648)-- (23.566939939701516,-12.956034869798504);
\draw [line width=2pt,color=zzttqq] (23.566939939701516,-12.956034869798504)-- (25.255595790705538,-11.884381279840516);
\draw [line width=2pt,color=zzttqq] (25.255595790705538,-11.884381279840516)-- (26.796622276257118,-10.609533300343136);
\draw [line width=2pt,color=zzttqq] (26.796622276257118,-10.609533300343136)-- (28.165716488114484,-9.151596045500321);
\draw [line width=2pt,color=zzttqq] (28.165716488114484,-9.151596045500321)-- (29.34128699269943,-7.533562056750428);
\draw [line width=2pt,color=zzttqq] (29.34128699269943,-7.533562056750428)-- (30.30479434090286,-5.780948696662704);
\draw [line width=2pt,color=zzttqq] (30.30479434090286,-5.780948696662704)-- (31.041043446272212,-3.9213957248862084);
\draw [line width=2pt,color=zzttqq] (31.041043446272212,-3.9213957248862084)-- (31.538423220601924,-1.9842294026289484);
\draw [line width=2pt,color=zzttqq] (31.538423220601924,-1.9842294026289484)-- (31.78908968773053,0);
\draw [line width=2pt,color=zzttqq] (31.78908968773053,0)-- (31.78908968773053,2);
\draw [line width=2pt,color=zzttqq] (31.78908968773053,2)-- (31.53842322060192,3.9842294026289498);
\draw [line width=2pt,color=zzttqq] (31.53842322060192,3.9842294026289498)-- (31.041043446272212,5.92139572488621);
\draw [line width=2pt,color=zzttqq] (31.041043446272212,5.92139572488621)-- (30.30479434090286,7.780948696662704);
\draw [line width=2pt,color=zzttqq] (30.30479434090286,7.780948696662704)-- (29.34128699269943,9.53356205675043);
\draw [line width=2pt,color=zzttqq] (29.34128699269943,9.53356205675043)-- (28.16571648811449,11.151596045500318);
\draw [line width=2pt,color=zzttqq] (28.16571648811449,11.151596045500318)-- (26.796622276257114,12.609533300343138);
\draw [line width=2pt,color=zzttqq] (26.796622276257114,12.609533300343138)-- (25.255595790705538,13.884381279840516);
\draw [line width=2pt,color=zzttqq] (25.255595790705538,13.884381279840516)-- (23.56693993970151,14.956034869798508);
\draw [line width=2pt,color=zzttqq] (23.56693993970151,14.956034869798508)-- (21.757285834769483,15.807593452928646);
\draw [line width=2pt,color=zzttqq] (21.757285834769483,15.807593452928646)-- (19.85517280217918,16.425627441678543);
\draw [line width=2pt,color=zzttqq] (19.85517280217918,16.425627441678543)-- (17.890598300721802,16.80039007084999);
\draw [line width=2pt,color=zzttqq] (17.890598300721802,16.80039007084999)-- (15.894544843865262,16.925971109908616);
\draw [line width=2pt,color=zzttqq] (15.894544843865262,16.925971109908616)-- (13.898491387008722,16.80039007084999);
\draw [line width=2pt,color=zzttqq] (13.898491387008722,16.80039007084999)-- (11.93391688555136,16.425627441678543);
\draw [line width=2pt,color=zzttqq] (11.93391688555136,16.425627441678543)-- (10.031803852961055,15.80759345292865);
\draw [line width=2pt,color=zzttqq] (10.031803852961055,15.80759345292865)-- (8.222149748029018,14.956034869798504);
\draw [line width=2pt,color=zzttqq] (8.222149748029018,14.956034869798504)-- (6.533493897024989,13.884381279840513);
\draw [line width=2pt,color=zzttqq] (6.533493897024989,13.884381279840513)-- (4.992467411473411,12.609533300343134);
\draw [line width=2pt,color=zzttqq] (4.992467411473411,12.609533300343134)-- (3.6233731996160383,11.151596045500312);
\draw [line width=2pt,color=zzttqq] (3.6233731996160383,11.151596045500312)-- (2.4478026950311005,9.53356205675043);
\draw [line width=2pt,color=zzttqq] (2.4478026950311005,9.53356205675043)-- (1.48429534682767,7.780948696662706);
\draw [line width=2pt,color=zzttqq] (1.48429534682767,7.780948696662706)-- (0.7480462414583151,5.921395724886204);
\draw [line width=2pt,color=zzttqq] (0.7480462414583151,5.921395724886204)-- (0.25066646712860674,3.9842294026289435);
\draw [line width=2pt,color=zzttqq] (0.25066646712860674,3.9842294026289435)-- (0,2);
\draw [line width=2pt] (31.78908968773053,0)-- (0,0);
\draw [line width=2pt] (15.894544843865262,16.925971109908616)-- (15.894544843865264,-14.925971109908616);
\begin{scriptsize}
\draw [fill=ududff] (0,2) circle (2.5pt);
\draw[color=ududff] (0.42462465041968367,3.132644907312989) node {$E$};
\draw [fill=ududff] (0,0) circle (2.5pt);
\draw[color=ududff] (0.42462465041968367,1.1421247832323964) node {$F$};
\draw [fill=uuuuuu] (0.2506664671286085,-1.9842294026289462) circle (2.5pt);
\draw[color=uuuuuu] (0.6865351930618673,-0.8483953408481963) node {$G$};
\draw [fill=uuuuuu] (0.7480462414583151,-3.921395724886205) circle (2.5pt);
\draw[color=uuuuuu] (1.1579741698177979,-2.7865333564003527) node {$H$};
\draw [fill=uuuuuu] (1.4842953468276683,-5.780948696662703) circle (2.5pt);
\draw[color=uuuuuu] (1.8913236892159118,-4.672289263424072) node {$I$};
\draw [fill=uuuuuu] (2.447802695031097,-7.5335620567504264) circle (2.5pt);
\draw[color=uuuuuu] (2.8865837512562096,-6.400898844862482) node {$J$};
\draw [fill=uuuuuu] (3.62337319961604,-9.151596045500318) circle (2.5pt);
\draw[color=uuuuuu] (4.038990138881817,-8.024744209244016) node {$K$};
\draw [fill=uuuuuu] (4.992467411473415,-10.609533300343136) circle (2.5pt);
\draw[color=uuuuuu] (5.400924960621172,-9.491443248040245) node {$L$};
\draw [fill=uuuuuu] (6.533493897024991,-11.884381279840513) circle (2.5pt);
\draw[color=uuuuuu] (6.972388216474274,-10.748613852722723) node {$M$};
\draw [fill=uuuuuu] (8.222149748029015,-12.956034869798504) circle (2.5pt);
\draw[color=uuuuuu] (8.648615689384249,-11.848638131819893) node {$N$};
\draw [fill=uuuuuu] (10.03180385296105,-13.807593452928646) circle (2.5pt);
\draw[color=uuuuuu] (10.429607379351097,-12.686751868274879) node {$O$};
\draw [fill=uuuuuu] (11.933916885551353,-14.425627441678541) circle (2.5pt);
\draw[color=uuuuuu] (12.367745394903256,-13.315337170616118) node {$P$};
\draw [fill=uuuuuu] (13.898491387008725,-14.80039007084999) circle (2.5pt);
\draw[color=uuuuuu] (14.305883410455413,-13.682011930315177) node {$Q$};
\draw [fill=uuuuuu] (15.894544843865264,-14.925971109908616) circle (2.5pt);
\draw[color=uuuuuu] (16.296403534536008,-13.786776147372048) node {$R$};
\draw [fill=uuuuuu] (17.890598300721805,-14.80039007084999) circle (2.5pt);
\draw[color=uuuuuu] (18.286923658616605,-13.682011930315177) node {$S$};
\draw [fill=uuuuuu] (19.855172802179176,-14.425627441678543) circle (2.5pt);
\draw[color=uuuuuu] (20.277443782697198,-13.315337170616118) node {$T$};
\draw [fill=uuuuuu] (21.757285834769476,-13.807593452928648) circle (2.5pt);
\draw[color=uuuuuu] (22.163199689720923,-12.686751868274879) node {$U$};
\draw [fill=uuuuuu] (23.566939939701516,-12.956034869798504) circle (2.5pt);
\draw[color=uuuuuu] (23.996573488216207,-11.848638131819893) node {$V$};
\draw [fill=uuuuuu] (25.255595790705538,-11.884381279840516) circle (2.5pt);
\draw[color=uuuuuu] (25.672800961126182,-10.748613852722723) node {$W$};
\draw [fill=uuuuuu] (26.796622276257118,-10.609533300343136) circle (2.5pt);
\draw[color=uuuuuu] (27.191882108450848,-9.491443248040245) node {$Z$};
\draw [fill=uuuuuu] (28.165716488114484,-9.151596045500321) circle (2.5pt);
\draw[color=uuuuuu] (28.763345364303948,-7.867597883658707) node {$A_1$};
\draw [fill=uuuuuu] (29.34128699269943,-7.533562056750428) circle (2.5pt);
\draw[color=uuuuuu] (29.915751751929555,-6.243752519277172) node {$B_1$};
\draw [fill=uuuuuu] (30.30479434090286,-5.780948696662704) circle (2.5pt);
\draw[color=uuuuuu] (30.858629705441416,-4.515142937838762) node {$C_1$};
\draw [fill=uuuuuu] (31.041043446272212,-3.9213957248862084) circle (2.5pt);
\draw[color=uuuuuu] (31.59197922483953,-2.629387030815043) node {$D_1$};
\draw [fill=uuuuuu] (31.538423220601924,-1.9842294026289484) circle (2.5pt);
\draw[color=uuuuuu] (32.1158003101239,-0.6912490152628864) node {$E_1$};
\draw [fill=uuuuuu] (31.78908968773053,0) circle (2.5pt);
\draw[color=uuuuuu] (32.377710852766086,1.2992711088177065) node {$F_1$};
\draw [fill=uuuuuu] (31.78908968773053,2) circle (2.5pt);
\draw[color=uuuuuu] (32.377710852766086,3.289791232898299) node {$G_1$};
\draw [fill=uuuuuu] (31.53842322060192,3.9842294026289498) circle (2.5pt);
\draw[color=uuuuuu] (32.1158003101239,5.280311356978892) node {$H_1$};
\draw [fill=uuuuuu] (31.041043446272212,5.92139572488621) circle (2.5pt);
\draw[color=uuuuuu] (31.59197922483953,7.218449372531048) node {$I_1$};
\draw [fill=uuuuuu] (30.30479434090286,7.780948696662704) circle (2.5pt);
\draw[color=uuuuuu] (30.858629705441416,9.051823171026331) node {$J_1$};
\draw [fill=uuuuuu] (29.34128699269943,9.53356205675043) circle (2.5pt);
\draw[color=uuuuuu] (29.915751751929555,10.832814860993176) node {$K_1$};
\draw [fill=uuuuuu] (28.16571648811449,11.151596045500318) circle (2.5pt);
\draw[color=uuuuuu] (28.763345364303948,12.456660225374714) node {$L_1$};
\draw [fill=uuuuuu] (26.796622276257114,12.609533300343138) circle (2.5pt);
\draw[color=uuuuuu] (27.349028434036157,13.870977155642503) node {$M_1$};
\draw [fill=uuuuuu] (25.255595790705538,13.884381279840516) circle (2.5pt);
\draw[color=uuuuuu] (25.82994728671149,15.18052986885342) node {$N_1$};
\draw [fill=uuuuuu] (23.56693993970151,14.956034869798508) circle (2.5pt);
\draw[color=uuuuuu] (24.153719813801516,16.22817203942215) node {$O_1$};
\draw [fill=uuuuuu] (21.757285834769483,15.807593452928646) circle (2.5pt);
\draw[color=uuuuuu] (22.32034601530623,17.066285775877137) node {$P_1$};
\draw [fill=uuuuuu] (19.85517280217918,16.425627441678543) circle (2.5pt);
\draw[color=uuuuuu] (20.434590108282507,17.694871078218377) node {$Q_1$};
\draw [fill=uuuuuu] (17.890598300721802,16.80039007084999) circle (2.5pt);
\draw[color=uuuuuu] (18.444069984201914,18.061545837917436) node {$R_1$};
\draw [fill=uuuuuu] (15.894544843865262,16.925971109908616) circle (2.5pt);
\draw[color=uuuuuu] (16.453549860121317,18.218692163502745) node {$S_1$};
\draw [fill=uuuuuu] (13.898491387008722,16.80039007084999) circle (2.5pt);
\draw[color=uuuuuu] (14.463029736040724,18.061545837917436) node {$T_1$};
\draw [fill=uuuuuu] (11.93391688555136,16.425627441678543) circle (2.5pt);
\draw[color=uuuuuu] (12.524891720488567,17.694871078218377) node {$U_1$};
\draw [fill=uuuuuu] (10.031803852961055,15.80759345292865) circle (2.5pt);
\draw[color=uuuuuu] (10.586753704936408,17.066285775877137) node {$V_1$};
\draw [fill=uuuuuu] (8.222149748029018,14.956034869798504) circle (2.5pt);
\draw[color=uuuuuu] (8.80576201496956,16.22817203942215) node {$W_1$};
\draw [fill=uuuuuu] (6.533493897024989,13.884381279840513) circle (2.5pt);
\draw[color=uuuuuu] (7.129534542059584,15.18052986885342) node {$Z_1$};
\draw [fill=uuuuuu] (4.992467411473411,12.609533300343134) circle (2.5pt);
\draw[color=uuuuuu] (5.5580712862064825,13.870977155642503) node {$A_2$};
\draw [fill=uuuuuu] (3.6233731996160383,11.151596045500312) circle (2.5pt);
\draw[color=uuuuuu] (4.196136464467127,12.456660225374714) node {$B_2$};
\draw [fill=uuuuuu] (2.4478026950311005,9.53356205675043) circle (2.5pt);
\draw[color=uuuuuu] (3.04373007684152,10.832814860993176) node {$C_2$};
\draw [fill=uuuuuu] (1.48429534682767,7.780948696662706) circle (2.5pt);
\draw[color=uuuuuu] (2.048470014801222,9.051823171026331) node {$D_2$};
\draw [fill=uuuuuu] (0.7480462414583151,5.921395724886204) circle (2.5pt);
\draw[color=uuuuuu] (1.315120495403108,7.218449372531048) node {$E_2$};
\draw [fill=uuuuuu] (0.25066646712860674,3.9842294026289435) circle (2.5pt);
\draw[color=uuuuuu] (0.8436815186471773,5.280311356978892) node {$F_2$};
\draw[color=black] (16.08687510042226,1.4564174344030163) node {$f$};
\draw[color=black] (15.248761363967274,1.6135637599883264) node {$c$};
\draw [fill=uuuuuu] (15.894544843865262,0) circle (2pt);
\draw[color=uuuuuu] (16.296403534536008,1.037360566175523) node {$A$};
\end{scriptsize}
\end{axis}
\label{setup}
\end{tikzpicture}

==> Source/Archi-arcface.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{darkslategray66}{RGB}{66,66,66}
\definecolor{lightgray}{RGB}{211,211,211}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{peru22412844}{RGB}{224,128,44}
\definecolor{steelblue49115161}{RGB}{49,115,161}

\begin{axis}[
axis background/.style={fill=none},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick align=outside,
unbounded coords=jump,
x grid style={lightgray},
xlabel={Model},
xmajorgrids,
xmajorticks=false,
xmajorticks=true,
xmin=-0.5, xmax=1.5,
xtick pos=lower,
xtick style={color=black},
xtick={0,1},
xticklabels={Crossentropy,Arcface},
y grid style={lightgray},
ylabel=\textcolor{darkslategray38}{TPR for a FPR of 0.1\%},
ymajorgrids,
ymajorticks=false,
ymajorticks=true,
ymin=0, ymax=22.1290198926236,
ytick pos=left,
ytick style={color=darkslategray38},
ytick={0,2.5,5,7.5,10,12.5,15,17.5,20,22.5},
yticklabels={
  \(\displaystyle {0.0}\),
  \(\displaystyle {2.5}\),
  \(\displaystyle {5.0}\),
  \(\displaystyle {7.5}\),
  \(\displaystyle {10.0}\),
  \(\displaystyle {12.5}\),
  \(\displaystyle {15.0}\),
  \(\displaystyle {17.5}\),
  \(\displaystyle {20.0}\),
  \(\displaystyle {22.5}\)
}
]
\draw[draw=black,fill=steelblue49115161,line width=0.32pt] (axis cs:-0.4,0) rectangle (axis cs:0,14.4633026163998);
\draw[draw=black,fill=steelblue49115161,line width=0.32pt] (axis cs:0.6,0) rectangle (axis cs:1,19.6848926377196);
\draw[draw=black,fill=peru22412844,line width=0.32pt] (axis cs:5.55111512312578e-17,0) rectangle (axis cs:0.4,19.7880350651267);
\draw[draw=black,fill=peru22412844,line width=0.32pt] (axis cs:1,0) rectangle (axis cs:1.4,21.0752570405939);
\draw[draw=black,fill=steelblue49115161,line width=0.32pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=black,fill=steelblue49115161,line width=0.32pt}
\addlegendentry{CNN}

\draw[draw=black,fill=peru22412844,line width=0.32pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=black,fill=peru22412844,line width=0.32pt}
\addlegendentry{ViT}

\addplot [line width=0.72pt, darkslategray66, forget plot]
table {%
-0.2 nan
-0.2 nan
};
\addplot [line width=0.72pt, darkslategray66, forget plot]
table {%
0.8 nan
0.8 nan
};
\addplot [line width=0.72pt, darkslategray66, forget plot]
table {%
0.2 nan
0.2 nan
};
\addplot [line width=0.72pt, darkslategray66, forget plot]
table {%
1.2 nan
1.2 nan
};
\end{axis}

\end{tikzpicture}


==> Source/Archi-input-type.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{brown1926061}{RGB}{192,60,61}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{darkslategray66}{RGB}{66,66,66}
\definecolor{lightgray}{RGB}{211,211,211}
\definecolor{peru22412844}{RGB}{224,128,44}
\definecolor{seagreen5814558}{RGB}{58,145,58}
\definecolor{steelblue49115161}{RGB}{49,115,161}

\begin{axis}[
axis background/.style={fill=none},
tick align=outside,
tick align=outside,
x grid style={lightgray},
xlabel={Input data type},
xmajorgrids,
xmajorticks=false,
xmajorticks=true,
xmin=-0.5, xmax=3.5,
xtick pos=lower,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={I/Q, I, Q, Magnitude},
y grid style={lightgray},
ylabel=\textcolor{darkslategray38}{CF1 score},
ymajorgrids,
ymajorticks=false,
ymajorticks=true,
ymin=0, ymax=0.6299004226769,
ytick pos=left,
ytick style={color=darkslategray38},
ytick={0,0.1,0.2,0.3,0.4,0.5,0.6,0.7},
yticklabels={
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.1}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.3}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.5}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.7}\)
}
]
\draw[draw=black,fill=steelblue49115161,line width=0.32pt] (axis cs:-0.4,0) rectangle (axis cs:0.4,0.573548488322573);
\draw[draw=black,fill=peru22412844,line width=0.32pt] (axis cs:0.6,0) rectangle (axis cs:1.4,0.469870582605019);
\draw[draw=black,fill=seagreen5814558,line width=0.32pt] (axis cs:1.6,0) rectangle (axis cs:2.4,0.424829751673606);
\draw[draw=black,fill=brown1926061,line width=0.32pt] (axis cs:2.6,0) rectangle (axis cs:3.4,0.465476673110411);
\addplot [line width=0.72pt, darkslategray66]
table {%
0 0.547191812190955
0 0.599905164454191
};
\addplot [line width=0.72pt, darkslategray66]
table {%
1 0.456625624992091
1 0.483115540217948
};
\addplot [line width=0.72pt, darkslategray66]
table {%
2 0.404039702782972
2 0.44561980056424
};
\addplot [line width=0.72pt, darkslategray66]
table {%
3 0.420237235367296
3 0.510716110853526
};
\end{axis}

\end{tikzpicture}


==> Source/Archi-preprocessing.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{darkslategray66}{RGB}{66,66,66}
\definecolor{lightgray}{RGB}{211,211,211}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{peru22412844}{RGB}{224,128,44}
\definecolor{steelblue49115161}{RGB}{49,115,161}

\begin{axis}[
axis background/.style={fill=none},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.5,0.91)},
  anchor=north,
  draw=lightgray204
},
tick align=outside,
tick align=outside,
unbounded coords=jump,
x grid style={lightgray},
xlabel={Preprocessing},
xmajorgrids,
xmajorticks=false,
xmajorticks=true,
xmin=-0.5, xmax=2.5,
xtick pos=lower,
xtick style={color=black},
xtick={0,1,2},
xticklabels={IQ,FFT,STFT},
y grid style={lightgray},
ylabel=\textcolor{darkslategray38}{CF1 score},
ymajorgrids,
ymajorticks=false,
ymajorticks=true,
ymin=0, ymax=0.702770588902536,
ytick pos=left,
ytick style={color=darkslategray38},
ytick={0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8},
yticklabels={
  \(\displaystyle {0.0}\),
  \(\displaystyle {0.1}\),
  \(\displaystyle {0.2}\),
  \(\displaystyle {0.3}\),
  \(\displaystyle {0.4}\),
  \(\displaystyle {0.5}\),
  \(\displaystyle {0.6}\),
  \(\displaystyle {0.7}\),
  \(\displaystyle {0.8}\)
}
]
\draw[draw=black,fill=steelblue49115161,line width=0.32pt] (axis cs:-0.4,0) rectangle (axis cs:0,0.580675739283908);
\draw[draw=black,fill=steelblue49115161,line width=0.32pt] (axis cs:0.6,0) rectangle (axis cs:1,0.507385469982387);
\draw[draw=black,fill=steelblue49115161,line width=0.32pt] (axis cs:1.6,0) rectangle (axis cs:2,0.655718203682815);
\draw[draw=black,fill=peru22412844,line width=0.32pt] (axis cs:5.55111512312578e-17,0) rectangle (axis cs:0.4,0.61051911580444);
\draw[draw=black,fill=peru22412844,line width=0.32pt] (axis cs:1,0) rectangle (axis cs:1.4,0.415894812997012);
\draw[draw=black,fill=peru22412844,line width=0.32pt] (axis cs:2,0) rectangle (axis cs:2.4,0.66930532276432);
\draw[draw=black,fill=steelblue49115161,line width=0.32pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=black,fill=steelblue49115161,line width=0.32pt}
\addlegendentry{CNN}

\draw[draw=black,fill=peru22412844,line width=0.32pt] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar,ybar legend,draw=black,fill=peru22412844,line width=0.32pt}
\addlegendentry{ViT}

\addplot [line width=0.72pt, darkslategray66, forget plot]
table {%
-0.2 nan
-0.2 nan
};
\addplot [line width=0.72pt, darkslategray66, forget plot]
table {%
0.8 nan
0.8 nan
};
\addplot [line width=0.72pt, darkslategray66, forget plot]
table {%
1.8 nan
1.8 nan
};
\addplot [line width=0.72pt, darkslategray66, forget plot]
table {%
0.2 nan
0.2 nan
};
\addplot [line width=0.72pt, darkslategray66, forget plot]
table {%
1.2 nan
1.2 nan
};
\addplot [line width=0.72pt, darkslategray66, forget plot]
table {%
2.2 nan
2.2 nan
};
\end{axis}

\end{tikzpicture}


==> Source/architecture_with_table.tex <==
% \usetikzlibrary{positioning}
\begin{figure}[h]
    \centering
    \begin{subfigure}[ht]{0.35\textwidth}
        \resizebox{0.4\textwidth}{!}{
            \begin{tikzpicture}[node distance=0.5cm and 2.5cm, >=latex, scale=0.6]
                %\pgflowlevelsynccm
                % Input layer
                \node (input) [draw, fill=red!20] {\textbf{Input}};
                % Convolutional layer 1
                \node (conv1) [below=of input, draw, fill=blue!20, text width=2.5cm, align=center] {Convolutional \\ Layer \\ $5 \times 5 \times 256 $};
                % Max pooling layer 1
                \node (pool1) [below=of conv1, draw, fill=green!20, text width=2.5cm, align=center] {Max Pooling \\ Layer};
                % Convolutional layer 2
                \node (conv2) [below=of pool1, draw, fill=blue!20, text width=2.5cm, align=center] {Convolutional \\ Layer};
                % Max pooling layer 2
                \node (pool2) [below=of conv2, draw, fill=green!20, text width=2.5cm, align=center] {Max Pooling \\ Layer};
                % Flatten layer
                \node (flatten) [below=of pool2, draw, fill=gray!20, text width=2cm, align=center] {Flatten};
                % Fully connected layer 1
                \node (fc1) [below=of flatten, draw, fill=yellow!20, text width=3cm, align=center] {Fully Connected \\ Layer};
                % Latent representation
                \node (Latent representation) [below=of fc1, draw, fill=red!20] {\textbf{Latent representation}};
                % Fully connected layer 2
                \node (fc2) [below=of Latent representation, draw, fill=yellow!20, text width=3cm, align=center] {Fully Connected \\ Layer};
                % Output layer
                \node (output) [below=of fc2, draw, fill=red!20] {\textbf{Output}};
                % Arrows
                \foreach \i in {conv1, pool1, conv2, pool2, flatten, fc1}
                    \draw[->] (input) -- (conv1);
                    \draw[->] (conv1) -- (pool1);
                    \draw[->] (pool1) -- (conv2);
                    \draw[->] (conv2) -- (pool2);
                \draw[->] (pool2) -- (flatten);
                \draw[->] (flatten) -- (fc1);
                \draw[->] (fc1) -- (Latent representation);
                \draw[->] (Latent representation) -- (fc2);
                \draw[->] (fc2) -- (output);
            \end{tikzpicture}
         }
        \caption{Convolutional Neural Network Structure}
    \end{subfigure}\hfill%
    % \begin{subfigure}[ht]{0.1\textwidth}
    %     \centering
    %     \begin{tabularx}{\textwidth}{|c|X|X|}
    %         \hline
    %         \textbf{Parameters} & \textbf{1D} & \textbf{2D} \\
    %         \hline
    %         \textbf{1. Convolutional Layer} & &\\
    %         Convolutional Features & 20 & 20\\
    %         Convolutional Kernel & \textbf{15} & \textbf{3}\\
    %         Stride Size & 2 & 2\\
    %         Padding Size & \textbf{7} & \textbf{1}\\
    %         \hline
    %         \textbf{1. Max Pooling Layer} & & \\
    %         Kernnel Size & 2 & 2\\
    %         Stride Size & 2 & 2\\
    %         \hline
    %         \textbf{2. Convolutional Layer} & &\\
    %         Convolutional Features & 20 & 20\\
    %         Convolutional Kernel & \textbf{15} & \textbf{3}\\
    %         Stride Size & 2 & 2\\
    %         Padding Size & \textbf{7} & \textbf{1}\\
    %         \hline
    %         \textbf{2. Max Pooling Layer} & & \\
    %         Kernnel Size & 2 & 2\\
    %         Stride Size & 2 & 2\\
    %         \hline
    %         \textbf{1. Fully Connected Layer} & &\\
    %         Output Dimension & 128 & 128\\
    %         \hline
    %         \textbf{2. Fully Connected Layer} & &\\
    %         Output Dimension & 13 & 13\\

    %         \hline
    %     \end{tabularx}
    % \caption{Convolutional Neural Network Parameters}
    % \end{subfigure}
    \caption{Convolutional Neural Network Architecture}
    \label{fig:cnn_model}
\end{figure}

==> Source/triple_figure_with_deviation.tex <==
\begin{figure}[htbp]
\hspace*{-2cm}
        \begin{subfigure}[ht]{.6\textwidth} % this sets the figure to be max half the width of the page
            %\centering
\pgfplotsset{compat=newest}
\begin{tikzpicture}
    \begin{axis}[
        %width  = 0.85*\textwidth,
        %height = 8cm,
        major x tick style = transparent,
        %ybar=2*\pgflinewidth,
        ybar,
        bar width=30pt,
        ymajorgrids = true,
        ylabel = {F1-Score},
        symbolic x coords={I,Q,Mag,IQ},
        xtick = data,
        nodes near coords, % this command is used to mention the y-axis points on the top of the particular bar.  
        nodes near coords style={anchor=south, yshift=11pt}, % Adjust the vertical offset here
        nodes near coords align={vertical}, 
        scaled y ticks = false,
        enlarge x limits=0.25,
        ymin=0,
        legend cell align=left,
        legend style={
                at={(1,1.05)},
                anchor=south east,
                column sep=1ex
        }
    ]
        \addplot[style={black,fill=bblue,mark=none},
                error bars/.cd,
                y dir=both,
                y explicit]
            coordinates {
            (I, 0.4402) -= (0,0.0794) +=(0, 0.0518) (Q, 0.4440) -= (0,0.0367) +=(0,0.0400) (Mag,0.4109) -= (0,0.0666) +=(0, 0.0398) 
            (IQ, 0.5582) -= (0,0.0480) +=(0, 0.0557)};
    \end{axis}
\end{tikzpicture}
\caption{F1-Score}
             
            
        \end{subfigure}
        \begin{subfigure}[ht]{.6\textwidth}
            \pgfplotsset{compat=newest}
\begin{tikzpicture}
    \begin{axis}[
        %width  = 0.85*\textwidth,
        %height = 8cm,
        major x tick style = transparent,
        %ybar=2*\pgflinewidth,
        ybar,
        bar width=30pt,
        ymajorgrids = true,
        ylabel = {Re-Identifikationsmetrik (\%)},
        symbolic x coords={I,Q,Mag,IQ},
        xtick = data,
        nodes near coords, % this command is used to mention the y-axis points on the top of the particular bar.  
        nodes near coords style={anchor=south, yshift=6pt}, % Adjust the vertical offset here
        nodes near coords align={vertical}, 
        scaled y ticks = false,
        enlarge x limits=0.25,
        ymin=0,
        legend cell align=left,
        legend style={
                at={(1,1.05)},
                anchor=south east,
                column sep=1ex
        }
    ]
        \addplot[style={black,fill=bblue,mark=none},
                error bars/.cd,
                y dir=both,
                y explicit]
            coordinates {
            (I, 43.04) -= (0,5.63) +=(0, 2.20) 
            (Q, 42.87) -= (0,3.61) +=(0, 3.49) (Mag,42.63) -= (0,3.37) +=(0, 4.01) (IQ,56.47) -= (0,1.91) +=(0, 1.93)};
    \end{axis}
\end{tikzpicture}
\caption{Re-Identifikationsmetrik}
        \end{subfigure}
        
        \begin{subfigure}[h]{\textwidth}

            \centering
            \begin{tikzpicture}
    \begin{axis}[
        %width  = 0.85*\textwidth,
        %height = 8cm,
        major x tick style = transparent,
        %ybar=2*\pgflinewidth,
        ybar,
        bar width=30pt,
        ymajorgrids = true,
        ylabel = {Area under ROC-Curve},
        symbolic x coords={I,Q,Mag,IQ},
        xtick = data,
        nodes near coords, % this command is used to mention the y-axis points on the top of the particular bar.  
        nodes near coords style={anchor=south, yshift=5pt}, % Adjust the vertical offset here
        nodes near coords align={vertical}, 
        scaled y ticks = false,
        enlarge x limits=0.25,
        ymin=0,
        legend cell align=left,
        legend style={
                at={(1,1.05)},
                anchor=south east,
                column sep=1ex
        }
    ]
        \addplot[style={black,fill=bblue,mark=none},
                error bars/.cd,
                y dir=both,
                y explicit]
            coordinates {
            (I, 0.7692) -= (0,0.0175) +=(0, 0.0175) (Q, 0.7682) -=(0,0.0164) +=(0, 0.0231)
            (Mag, 0.8144) -=(0,0.0237) +=(0, 0.0310) 
            (IQ, 0.8715) -=(0,0.0319) +=(0, 0.0280)};
    \end{axis}
\end{tikzpicture}
        \caption{Area under ROC-Curve basierend auf NN-Klassifizierung der Testdaten}
    \end{subfigure}
        \caption{Testmetriken für die drei verschiedenen Dateneingaben I-In-phase, Q-Quadrature, Mag-Magnitude und IQ-In-phase und Quadrature}
        \label{fig:experiment1}
\end{figure}
